BRAIN: Bias-Mitigation Continual Learning Approach to Vision-Brain Understanding

Memory decay makes it harder for the human brain to recognize visual objects and retain details. Consequently, recorded brain signals become weaker, uncertain, and contain poor visual context over time. This paper presents one of the first vision-learning approaches to address this problem. First, we statistically and experimentally demonstrate the existence of inconsistency in brain signals and its impact on the Vision-Brain Understanding (VBU) model. Our findings show that brain signal representations shift over recording sessions, leading to compounding bias, which poses challenges for model learning and degrades performance. Then, we propose a new Bias-Mitigation Continual Learning (BRAIN) approach to address these limitations. In this approach, the model is trained in a continual learning setup and mitigates the growing bias from each learning step. A new loss function named De-bias Contrastive Learning is also introduced to address the bias problem. In addition, to prevent catastrophic forgetting, where the model loses knowledge from previous sessions, the new Angular-based Forgetting Mitigation approach is introduced to preserve learned knowledge in the model. Finally, the empirical experiments demonstrate that our approach achieves State-of-the-Art (SOTA) performance across various benchmarks, surpassing prior and non-continual learning methods.

==> biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pics/bacnx.jpeg}}]{Xuan-Bac Nguyen}
is currently a Ph.D. student at the Department of Computer Science and Computer Engineering of the University of Arkansas. He received his M.Sc. degree in Computer Science from the Electrical and Computer Engineering Department at Chonnam National University, South Korea, in 2020.  He received his B.Sc. degree in Electronics and Telecommunications from the University of Engineering and Technology, VNU, in 2015. In 2016, he was a software engineer in Yokohama, Japan. His research interests include Quantum Machine Learning, Face Recognition, Facial Expression, and Medical Image Processing.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pics/dat.png}}]{Thanh-Dat Truong}
is currently a Postdoctoral Fellow at the University of Arkansas. He received his PhD degree from the University of Arkansas in 2024 and 
his B.Sc. degree in Computer Science from the University of Science (VNU) in 2019. He was a research intern at Coordinated Lab Science at the University of Illinois at Urbana-Champaign in 2018. 
Thanh-Dat Truong received the CVPR Doctoral Consortium Award in 2024.
His research aims to develop a robust and fair vision learning approach.
Truong's research interests include unsupervised domain adaptation, continual learning, action recognition, domain generalization, and deep generative models. His papers appear at top-tier conferences and journals such as CVPR, ICCV, NeurIPS, Neurocomputing, and ICPR.  He is also a reviewer of top-tier journals and conferences, including IEEE TPAMI, IEEE TIP, IEEE TAI, IEEE TCSVT, CVPR, ICCV, ECCV, ACCV, WACV, ICPR, ICML, ICLR, and NeurIPS.  
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pics/pawan.jpg}}]{Pawan Sinha} is a professor of neuroscience at MIT. Pawan’s research interests span brain science, AI, and public health. His experimental work involves studying healthy individuals and also those with neurological disorders such as autism. Pawan founded Project Prakash in 2005 with the twin objectives of providing treatment to children with severe visual impairments and also understanding mechanisms of learning and plasticity in the brain. This project has provided insights into several fundamental questions about brain function (even some that had remained open for the past three centuries) while also transforming the lives of many blind children by bringing them the gift of sight.
Pawan is a recipient of the PECASE – US Government’s highest award for young scientists, the Sloan Foundation Fellowship, and the Troland Award from the National Academies. He was inducted into the Guinness Book of World Records for creating the world’s smallest reproduction of a printed book.
\end{IEEEbiography}
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pics/khoa_luu.jpg}}]{Khoa Luu} is an Associate Professor and the Director of the Computer Vision and Image Understanding (CVIU) Lab in the Department of Computer Science \& Computer Engineering at the University of Arkansas, Fayetteville. He is affiliated with the Center for Public Health and Technology, UA, and the NSF MonARK Quantum Foundry. He is an Associate Editor of the Multimedia Tools and Applications Journal, Springer Nature. He is also the Area Chair in CVPR 2023-2025, NeurIPS 2024-25, WACV 2025, ICML 2025, ICLR 2025-2026, AAAI 2026 and Quantum Week 2025. He was the Research Project Director in the Cylab Biometrics Center at Carnegie Mellon University (CMU), USA. 
He received eight patents, three Best Paper awards, and co-authored over 120 papers in conferences, technical reports, and journals.
He was a vice chair of the Montreal Chapter IEEE SMCS in Canada from September 2009 to March 2011. His research interests include Computer Vision, Semantic Video Understanding, Biometrics, Face Recognition, Tracking, Human Behavior Understanding, Domain Adaptation, Deep Generative Modeling, Image and Video Processing, Compressed Sensing, and Quantum Machine Learning. 
He is a co-organizer and chair of the CVPR Precognition Workshop 2019-2025; the MICCAI Workshop in 2019, 2020, and the ICCV Workshop in 2021. He is a PC member of AAAI, ICPRAI in 2020 and 2022. 

\end{IEEEbiography}

